Beyond Matryoshka: Revisiting Sparse Coding for Adaptive Representation

Many large-scale systems rely on high-quality deep representations (embeddings) to facilitate tasks like retrieval, search, and generative modeling. Matryoshka Representation Learning (MRL) recently emerged as a solution for adaptive embedding lengths, but it requires full model retraining and suffers from noticeable performance degradations at short lengths. In this paper, we show that sparse coding offers a compelling alternative for achieving adaptive representation with minimal overhead and higher fidelity. We propose Contrastive Sparse Representation (CSR), a method that sparsifies pre-trained embeddings into a high-dimensional but selectively activated feature space. By leveraging lightweight autoencoding and task-aware contrastive objectives, CSR preserves semantic quality while allowing flexible, cost-effective inference at different sparsity levels. Extensive experiments on image, text, and multimodal benchmarks demonstrate that CSR consistently outperforms MRL in terms of both accuracy and retrieval speed-often by large margins-while also cutting training time to a fraction of that required by MRL. Our results establish sparse coding as a powerful paradigm for adaptive representation learning in real-world applications where efficiency and fidelity are both paramount. Code is available at https://github.com/neilwen987/CSR_Adaptive_Rep

==> sec/6_Discussions_and_Limitations.tex <==



% \subsection{Relationships with Other Acceleration Methods}
% In real-world deployment, leveraging deep representations involves two steps: (1) a computationally expensive forward pass to generate embeddings, and (2) downstream application of these embeddings. 
% Current methods like pruning~\cite{he2017channel}, quantization~\cite{jacob2018quantization}, and distillation~\cite{hinton2015distilling} enable accelerating the backbone and inference embedding generation (step 1).
% In contrast, our approach (CSR) focuses on post-processing optimization from embedding to retrieval (step 2). This \textbf{orthogonality} allows CSR to complement existing acceleration techniques for additional efficiency gains with minimal cost of performance.

% \subsection{Limitations}
% Like other sparsity-based methods, CSR suffers from the dead latent problem under extreme sparsity conditions, as discussed in Section~\ref{sec:SAE}. This issue is particularly pronounced in the multimodal domain, which we comprehensively examine in Section~\ref{sec:discuss_deat_lantent}.

% As a 2-layer MLP, CSR demonstrates consistent effectiveness across our experiments (even in zero-shot settings, see results from Table~\ref{table:mm_retrieval_result}) compared with MRL (fully fine-tuning).
% Further, we analyze the impact of different loss functions on the dead latent problem in Figure~\ref{fig:dead_dim}, where the incorporation of contrastive loss mitigates the dead latent issue.
% Based on these collections, we identify this phenomenon as a technical challenge requiring additional techniques (e.g., alternative loss function designs or deeper network architectures) to fully address.
